Offline Diversity Maximization Under Imitation Constraints

There has been significant recent progress in the area of unsupervised skill discovery, utilizing various information-theoretic objectives as measures of diversity. Despite these advances, challenges remain: current methods require significant online interaction, fail to leverage vast amounts of available task-agnostic data and typically lack a quantitative measure of skill utility. We address these challenges by proposing a principled offline algorithm for unsupervised skill discovery that, in addition to maximizing diversity, ensures that each learned skill imitates state-only expert demonstrations to a certain degree. Our main analytical contribution is to connect Fenchel duality, reinforcement learning, and unsupervised skill discovery to maximize a mutual information objective subject to KL-divergence state occupancy constraints. Furthermore, we demonstrate the effectiveness of our method on the standard offline benchmark D4RL and on a custom offline dataset collected from a 12-DoF quadruped robot for which the policies trained in simulation transfer well to the real robotic system.

==> commands.tex <==
\newcommand{\Real}{\ensuremath{\mathbb R}}        % Real numbers
\newcommand{\Unit}{\ensuremath{\mathbb I}}        % Unit Matrix
\newcommand{\T}{\ensuremath{\top}}                % Transpose
%\newcommand{\CharOver}[2]{\ensuremath{\overset{_{#1}}{#2}}}

\DeclareMathOperator*{\argmin}{arg\,min}   % the * make the subscript comes under the name of the operator
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\method}{MyMethod\xspace}

